Seeing Before Reasoning: Decoupling Perception and Reasoning for Shortcut-Resilient Multimodal On-Policy Self-Distillation

On-policy self-distillation (OPSD) trains a model on its own rollouts and uses a frozen copy to provide dense token-level targets conditioned on a reference target. This works well for LLM reasoning, but a direct extension to multimodal large language models (MLLMs) can create a shortcut: the privileged target may guide tokens mainly based on the text reference target rather than the image. We propose ViGOS, a visually grounded OPSD framework for MLLM post-training. The student first writes a visual description and then reasons toward the final answer. For valid rollouts, an image-only perception teacher supervises the description, while a privileged reasoning teacher supervises the reasoning and final answer on the same student prefix. A reference teacher is used only for invalid rollouts to recover the output format. Across general vision-language, expert reasoning, visual math, spatial grounding, and visual-language-prior benchmarks, ViGOS keeps the main benefits of OPSD and improves image-grounded behavior in shortcut-prone settings.

==> tables/main_algorithm.tex <==
\begin{algorithm}[t]
\caption{\method Training}
\small
\label{alg:ViGOS}
\begin{algorithmic}[1]
\REQUIRE Training set $\mathcal{D}$, student $p_\theta$, detached teacher parameters $\bar{\theta}$, and weights $\lambda_{\mathrm{perc}},\lambda_{\mathrm{rea}},\lambda_{\mathrm{ref}}$.
\FOR{each minibatch $(I,x,a^\star)$}
    \STATE Sample rollouts $y\sim p_\theta(\cdot\mid c_{\mathrm{stu}})$ from the student for the minibatch.
    \FOR{each rollout $y$ in the minibatch}
        \STATE Parse $y$ into $\mathcal{T}_d$, $\mathcal{T}_r$, $\mathcal{T}_a$, and $m_{\mathrm{inv}}(y)$; use empty segment masks if invalid.
        \IF{$m_{\mathrm{inv}}(y)=0$}
            \STATE Query $q_{\mathrm{img}}$ on student prefixes for $t\in\mathcal{T}_d$.
            \STATE Query $q_{\mathrm{rea}}$ on student prefixes for $t\in\mathcal{T}_r\cup\mathcal{T}_a$.
            \STATE Compute $\mathcal{L}_{\mathrm{perc}}$ and $\mathcal{L}_{\mathrm{rea}}$; set $\mathcal{L}_{\mathrm{ref}}=0$.
        \ELSE
            \STATE Query $q_{\mathrm{ref}}$ on student prefixes for $t\in\mathcal{T}_y$.
            \STATE Compute $\mathcal{L}_{\mathrm{ref}}$; set $\mathcal{L}_{\mathrm{perc}}=\mathcal{L}_{\mathrm{rea}}=0$.
        \ENDIF
    \ENDFOR
    \STATE Average the active losses over the minibatch, compute $\mathcal{L}_{\mathrm{ViGOS}}$, and update $\theta$.
\ENDFOR
\end{algorithmic}
\end{algorithm}

